The Emergence of Software Diversity in Maven Central

Maven artifacts are immutable: an artifact that is uploaded on Maven Central cannot be removed nor modified. The only way for developers to upgrade their library is to release a new version. Consequently, Maven Central accumulates all the versions of all the libraries that are published there, and applications that declare a dependency towards a library can pick any version. In this work, we hypothesize that the immutability of Maven artifacts and the ability to choose any version naturally support the emergence of software diversity within Maven Central. We analyze 1,487,956 artifacts that represent all the versions of 73,653 libraries. We observe that more than 30% of libraries have multiple versions that are actively used by latest artifacts. In the case of popular libraries, more than 50% of their versions are used. We also observe that more than 17% of libraries have several versions that are significantly more used than the other versions. Our results indicate that the immutability of artifacts in Maven Central does support a sustained level of diversity among versions of libraries in the repository.

==> old-text.tex <==
% space between paragraphs
% \vspace{0.25\baselineskip}

Different version instances of these libraries (\aka \textit{artifacts}) are ordered by version numbers.  We use an ordering function that considers the standard version numbering policy described by the Apache Maven foundation\footnote{\url{https://cwiki.apache.org/confluence/display/MAVEN/Version+number+policy}}. We denote this function by $\orderV$. Another core feature of Maven is the dependency management. Libraries versions are able to reuse existing libraries by adding a dependency to the Project Object Model (\texttt{pom.xml}) file, in the dependencies declaration section. In addition to the version numbers ordering, library versions in Maven can be also ordered in time. This order is prescribed by the timestamp at which a version was deployed on the repository. We denote this order function by $\orderT$. \looseness = -1




For the past 16 years, \mc have witnessed an exponential growth both in terms of the number of libraries and number of versions~\cite{Benelallam2019}. To assess the diversity and sustainability of this growth, we analyzed $1,487,956$ distinct versions of $73,653$ libraries coming from the \mdg dataset. To do so, we looked at the usage of every single library and version from different angles, activity status, popularity, and timeliness.




\subsection{Popularity in Maven Central}
We use two different metrics to measure the popularity of libraries and versions. One metric each.  It serves at ranking libraries or versions according to their connectivity and importance in the \mc. We recognized three different classes of popularity among libraries. Libraries with versions almost evenly popular, libraries with exactly one significantly popular version, and libraries with two or more significantly popular versions, sometimes belonging to different major versions. While the first class of libraries suggests that users do not favor any version over its peers, the third class of libraries indicates that niches of users are constructed around the most significantly popular versions. As we discussed previously, these versions may be part of two different major versions, reinforcing our hypothesis about the emerging diversity in \mc. Moreover, we observed that there is a strong correlation between the percentages of active versions and the popularity of the library. The higher the ratio of active versions in a library, the more likely it is to be popular.






\subsection{Data collection}

Data collection involved retrieving  \texttt{pom.xml} files (at least one per library version) from Maven Central, parsing them to retrieve metadata, and finally storing this information into a graph database. This a time-consuming process that we distributed  on top of a Docker Swarm cluster.
Figure~\ref{fig:architecture} shows the overall architecture and methodology. The process  ran on a cluster of 4 identical machines running an Ubuntu 18.04 LTS. Each machine has 16 Gb of RAM and 4 identical CPUs (MD A10-7700K APU with Radeon(TM) R7 Graphics, 2.105 GHz). One machine played the role of a Swarm Master while the others were Swarm Slaves.

\begin{figure}[htb]
\centering
 \includegraphics[width=.9\linewidth]{figures/architecture}
  \caption{Architecture used for mining Maven Central.}
  \label{fig:architecture}
\end{figure}

We rely on a producer-consumer pattern to distribute the computation (upper part of Figure~\ref{fig:architecture}). The producer is responsible for reading the Maven Central Index, wrapping artifact coordinates into messages, and publishing them in a shared messaging queue. On the other side, each consumer retrieves one artifact coordinate at a time. For each artifact, the consumer resolves the artifact's meta-data as well as its direct dependencies and store them in a graph database. Finally, the consumer acknowledges the broker having finished processing the message. In case of a consumer failure, the message broker puts back the message in the queue. Note messages are removed from the queue only if the corresponding consumer acknowledges so. Moreover, a message is processed by only one consumer at a time. When all artifacts are resolved, a post-processing phase is responsible for creating artifacts versions chains.\looseness=-1

For message queuing, we use RabbitMQ~\cite{rabbitmq}, a scalable and widely used message broker. As for the graph database backed, we rely on Neo4j~\cite{neo4j}, one of the most popular NoSQL databases. It comes along with a powerful SQL-like graph query language, Cypher~\cite{cypher}. This simplifies the exploitation of the dataset in a very simple manner. Finally, to fetch artifacts from Maven Central and resolve their direct dependencies, we use Aether~\cite{aether} Eclipse, a Java library to manage artifact repositories. 

Figure~\ref{fig:new_monthly_releases} shows in a y-logarithmic scale the number of new libraries as well as the number of library versions (in dashed lines) released each year in \mc until the \snapshot date. We observe that the number of new versions is greater than the number of new libraries, which indicates that developers use the repository not only to host but also to maintain their projects. Interestingly, there is a visible peak in the number of projects added to \mc on August 10, 2016. We suspect this is due to a massive deployment of an existing repository mirror on \mc, resulting in different release date for those libraries, which does not reflect their real availability date to the Java world.

\begin{figure}[htb]
	\centering  
	\includegraphics[origin=c,width=0.4\textwidth]{figures/new_yearly_releases.pdf}
	\caption{Yearly evolution of the number of new libraries and versions released in Maven Central.}
	\label{fig:new_monthly_releases}
\end{figure}

We observe an exponential grow over time with respect to the number of new libraries and the number of new versions deployed in \mc. To verify this, we performed a linear regression using an ordinary least square method on the logarithmic values. The adjusted $R^2$ values obtained were 0.85 and 0.8 for libraries and versions respectively, which confirm the hypothesis.

\subsection{\RQthree}

To answer our third research question, we investigate the upgrade behaviour of libraries. More specifically, we explore to what extent library maintainers rely on the latest available version when declaring their dependencies. Since the immutability of \mc allows them to choose among any of the existing dependency versions of a library, the determination of whether to keep such dependencies up to date or not through each new release is mostly a human-based choice. We use the newness metric to assess this behaviour.


From our dataset, we consider a total of 41,295 libraries which have at least one declared dependency. The total number of analyzed dependencies is 180,939. The 57.25\% of such libraries use updated dependencies, whereas the 42.74\% do not.

Figure~\ref{fig:outdated_dep} shows a violin plot with the distribution of the percentages of dependencies for all the libraries (i.e., percentage of outdated dependencies per library). We observe that most of the library maintainers rely in the latest available dependency version, with a median of outdated usage of 0\% and mean of 27.84\% (1st-Q and 3rd-Q corresponding to 0\% and 50\%, respectively).  

\begin{figure}[htb]
	\centering
	\includegraphics[origin=c,width=0.4\textwidth]{figures/outdated_dep.pdf}
	\caption{Distribution of libraries with outdated dependencies.}
	\label{fig:outdated_dep}
\end{figure}

Now we focus on characterizing and comparing the dependencies updating trend over time. Figure~\ref{fig:perc_out} shows the mean percentages of outdated dependencies in libraries from 2015 until our \snapshot of \mc. Interesting, as the linear regression suggest ($R^2 = 0.41$), we observe a steady significant increase (p-value = 0.01) in the adoption of outdated dependencies since the last decade. 

\begin{figure}[htb]
	\centering
	\includegraphics[origin=c,width=0.4\textwidth]{figures/perc_out.pdf}
	\caption{Yearly percentage of libraries with outdated dependencies.}
	\label{fig:perc_out}
\end{figure}

\begin{mdframed}[style=mpdframe]
\textbf{Findings from RQ3:} Developers are more inclined to adopt the latest released version of their declared dependencies. However, there is an increasing trend in recent years to keep using outdated but popular dependencies. 
\end{mdframed}

% This structure allows to obtain quantitative information about the repository using graph-based metrics, e.g., the most used artifacts, the path lengths of transitive dependencies, the degree distribution, clustering levels, and the presence of patterns. Our analysis was guided by the following objectives: (i) explore the global structure of Maven Central, (ii) analyze the degree of interrelation between artifacts, (iii) determine the most influential artifacts and (iv) describe the evolution of popular libraries.

%\mc is the largest and most used repository of JVM-based artifacts. It is mainly composed by a large collection of Java projects which are commonly deployed using the Maven dependency management system. In \mc, when a new artifact is released it becomes immutable, which means that it can not be either modified or removed from the repository. This immutability mechanism allows to maintain the stability of the system by preventing inconsistencies such as broken dependencies or backward incompatibilities. However, it also causes security problems by allowing the declaration and usage of outdated artifacts with known vulnerabilities. 

\amine{An upgrade aberration is when a library releases a new version without upgrading to latest dependencies.}

\amine{Def: An artifact validity period starts at its release date up to the release of the next version}

\nicolas{For traceability reasons other tools vendors would also deploy Nightly builds (back it up with evidences(numbers))}



% Software ecosystems are defined as ‘a collection of software  systems, which are developed and co-evolve in the same environment’ (Towards reverse engineering software ecosystems)

% software evolution has shifted to a macro-level, focusing on the evolution of large collections or distributions of software systems


%-----------------------------------------------------------------------------------------------------------

%Collections of OSS projects developed by the same developer community can be considered as software ecosystems bearing many similarities with biological ecosystems. While biological ecosystems have been the subject of study for many decades, research on software ecosystems is more recent. For this reason, this research project aim to determine whether and how selected ecological models and theories from biological ecosystems can be adapted and adopted to understand and better explain how OSS projects (akin to biological species) evolve, and to determine what are the main factors that drive the success or popularity of these projects. Expressed in biological terms, we wish to use knowledge on the evolution of biological ecosystems to provide support aiming to optimize the fitness, resistance and resilience of OSS projects. These insights will be implemented as guidelines in an evolution dashboard that helps to improve upon the daily practices of OSS communities.

%In an ecosystem, in contrast, many of its constituents depend on one another and therefore cannot function in isolation.

%Many researchers have started to study the analogies between biology (more specifically, ecology, biological evolution, and the dynamics of natural ecosystems) and software evolution [16,17]. The hope is that these analogies will lead to new insights, mechanisms, principles, and tools to improve software evolution.

%We will adopt these theories to study and model the evolution of OSS projects in their ecosystem of competing projects. 
%I draw an analogy between software ecosystems and natural ecosystems

In this paper, we interpreted the terminology and concepts used in software dependency management systems from an evolutionary point of view. The interaction among software artifacts deployed in Maven Central could be seen as a dynamic environment of evolving living organisms. In this context, each artifact is an individual. 

We build a taxonomic rank for Maven Central that distinguish the following hierarchy:

\begin{itemize}
	\item \textit{\textbf{Ecosystem:}}~The collection of all deployed projects which are developed and evolve in Maven Central.
	\item \textit{\textbf{Domain:}}~Two type of libraries, those used during testing or used at runtime.
	\item \textit{\textbf{Class:}}~Libraries that serve the same purpose or same category.
\end{itemize}

In Maven, an Artifacts is something that is either produced or used by a project. Artifacts are described by the 3-tuple "GroupId:ArtifactId:Version", distinguishing different versions of a given library ("GroupId:ArtifactId"). Library based rank:

\begin{itemize}
	\item \textit{\textbf{Family:}}~A group ID is a universally unique identifier for a project. While this is often just the project name (eg. commons-collections), it is helpful to use a fully-qualified package name to distinguish it from other projects with a similar name (eg. org.apache.maven).
	\item \textit{\textbf{Genus:}}~ArtifactID
	\item \textit{\textbf{Specie:}}~ A new release of an artifact that succeeds (i.e., corresponds to a higher version number or timestamp) a previous release of the same package.
\end{itemize}

As occurs in nature, the individuals of the same or of different species interact in its ecosystem. In Maven, we distinguish the following types of interactions:

\begin{itemize}
	\item \textit{\textbf{Dependency:}}~An explicitly documented reference (in the manifest of a release) to another package that is required for its proper functioning. A dependency can specify constraints to restrict the supported releases of the target package. Dependencies that are explicitly documented in the release manifest (i.e., edges in the dependency network) are called direct dependencies. Those that are part of the transitive closure of the dependency network are called transitive dependencies. Transitive dependencies that are not direct are called indirect dependencies.
	\item \textit{\textbf{Usage:}}~A package that is the target of at least one reverse dependency from another package. In a similar vein, we define transitively dependent.
\end{itemize}

% NOTE: Very related with the concept of symbiosis 



%In \mc, everything that is either produced or used by a software project is an \textit{artifact}. Each artifact is identified by a unique \textit{coordinates},  represented as a 3-tuple (groupId, artifactId, version). The set of different versions with similar groupId and artifactId are referred to as libraries and are represented as a couple (groupId, artifactId).
 %()We refer to all the versions of a given graph In this paper, we consider a \textit{library} to be a 2-tuple of G:A ("groupId:artifactId"). The set of artifacts with the same G:A represent different \textit{versions} of the library.
 
%The \mc repository can be represented as an unweighted directed graph, where vertices are artifacts and edges describe their relationships. Fig.~\ref{fig:graph_example} illustrates the different elements within a simplified graph $G$ with three libraries $\{A, B, C\}$ and seven artifacts $\{a_1, a_2, b_1, b_2, c_1, c_2, c_3\}$.

%More formally, let $G = (V, E)$ be the Maven Dependency Graph (MDG) with $V$ vertices (artifacts) and $E$ directed edges (dependency relationships). We distinguish between two different types of edges: $E_\text{\textit{depends}}$ and $E_\text{\textit{next}}$, with $E = E_\text{\textit{depends}} \cup E_\text{\textit{next}}$. The set $E_\text{\textit{depends}} = \{b \rightarrow a ~|~b \text{ has a direct dependency of } a\}$. The set $E_\text{\textit{next}} = \{a_1 \rightarrow a_2 ~|~a_2 \text{ is the next released version of library } A \text{ after } a_1\}$. 
%\amine{I would formalize my MDG as follows $G = (V, D, N)$ where $R$ is the set dependency relationships and $N$ the set of versions precedence }

%Artifacts can be self-contained~\footnote{\amine{we should explain self-contained with respect to what (I guess here you mean self-contained \wrt classpath and dependencies!)}} or depend on other artifacts. If an artifact $b$ depends on an artifact $a$, then we say that $b$ has a \textit{direct dependency} to $a$ (i.e. artifact $a$ is \textit{used} by $b$). Artifacts can have \textit{transitive dependencies}. If an artifact $c$ has a direct dependency to $b$, then $c$ has a transitive dependency to $a$. Transitive dependencies can be included through multiple levels of dependencies. In the MDG, a transitive dependency between $c$ and $a$, represented as $c \dashrightarrow a$ means that there is a path $c \rightarrow b \rightarrow ... \rightarrow a$ with length $> 1$ that connects $a$ and $c$ by edges of type $E_\text{\textit{depends}}$. 

% NOTE: Is there 'only' one popular? Are there dead versions?
% NOTE: Two fitness functions: (1) Based on the intuition that people should be upgrading to latest versions, we should expect at least usages from clients that have upgraded during project validity time that are still maintained, (2) Averaging the usages per G:A.

%We define that an artifact $a$ is \textit{alive} when it is the last version of a library or there is an artifact $b$ that is alive and it has a direct or transitive dependency with $a$. The artifacts that do not meet this definition are considered to be \textit{dead}. A dead library means that all their users migrated to new versions or started using another library instead. A vertices $a_i$ is considered as dead when there is a edge $a_i \rightarrow a_j$ of type $E_\text{\textit{next}}$ and $\nexists b \in V$ such as $b \dashrightarrow a_i$ or $b \rightarrow a_i$, being $b$ alive.












%To answer our last research question, we investigate the characteristics of the most successful libraries and versions in \mc. In order to determining the success of a released library, we rely on the fitness function defined in Section~\ref{sec:study_design}, i.e., to what degree the released versions satisfies the library clients. Accordingly, each new release is classified in one of the following three classes: Fit, Over-fit and Under-fit. Figure~\ref{fig:versions_timeliness} shows the distributions of library versions corresponding to each fitness class in our dataset. We notice that the 55\% of released versions fit the purpose ($fit(v) = 1$), while the 25\% over-fit. The remainder 20\% of the released versions belong to the under-fit class ($fit(v) < 1$). 

%We use a recursive partitioning tree in order to get insights about the rules that determine a version to success~\cite{Therneau1997:An_Introduction_to_Recursive_Partitioning_Using_the_RPART_Routines}. For our model, we consider the following variables: validity time, number of usages, passive or active, lifespan, PageRank, and number of dependencies. 
%Figure~\ref{fig:dt} depicts the decision tree obtained. Internal nodes are split according to the Gini index, terminal nodes represent the classification outcome and the probability of each class at that node. In the tree, we observe that the number of usages is the root node and, therefore, the most significant variable. According to the tree, versions with a number of usages greater or equal than two fit or over-fit, whereas versions with less than two usages depend on the validity time.

%The success of a library version is mostly determined by its number of usages. In general, versions with more than two direct usages have a high probability to be successful.

%\begin{figure}[htb]
%	\centering
%	\includegraphics[origin=c,width=0.45\textwidth]{figures/dt.pdf}
%	\caption{Decision tree of the fitting of library versions in \mc.}
%	\label{fig:dt}
%\end{figure}



==> tables/major.tex <==
\begin{table}[htb]
\centering
\caption{Distinct active major versions in libraries}
\begin{tabular}{cr} 
\toprule
\textbf{Major versions} & \textbf{Frequency} \\ 
\hline
$1$  &  $61,062$  \\
$2$  &  $7,418$ \\
$3$  &  $1,341$ \\ 
$4$  &  $308$ \\ 
$5$  &  $92$ \\ 
$6$  &  $44$ \\ 
$7$ &  $7$ \\ 
%\hline
%Total & XXX & XXX \\
\bottomrule
\label{tab:majors}
\end{tabular}
\end{table}

==> tables/stats.tex <==
\begin{table}[htb]
    \caption{Descriptive statistics of the libraries and versions in the Maven Dependency Graph}
    \centering
    \begin{tabular}{lccccc}
    \toprule
 \multirow{2}{*}{} & \multicolumn{1}{c}{} & \multicolumn{3}{c}{Quantiles} &  \\ 
\cline{3-5}
 & \multicolumn{1}{c}{Min} & \multicolumn{1}{c}{1st-Q} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{3st-Q} & Max \\
    \hline
    \#Library Versions & $1$ & $1$ & $10.77$ & $9$ & $2,183$   \\
    \#Library Usages & $0$ & $0$ & $43.47$ & $5$ & $251,836$  \\
    \#Library Dependencies & $0$ & $0$ & $43.47$ & $23$ & $35,149$ \\
    \#Version Usages & $0$ & $0$ & $4.16$ & $1$ & $47,951$ \\
    \#Version Dependencies & $0$ & $0$ & $4.12$ & $5$ & $402$ \\
    \bottomrule
    \end{tabular}
    \label{tab:evolution}
\end{table}

==> utils/utils.tex <==
\usepackage{soul}
\usepackage{tikz}

\usetikzlibrary{calc}
\usetikzlibrary{decorations.pathmorphing}


\makeatletter

\newcommand{\defhighlighter}[3][]{%
  \tikzset{every highlighter/.style={color=#2, fill opacity=#3, #1}}%
}

\defhighlighter{yellow}{.5}

\newcommand{\highlight@DoHighlight}{
  \fill [ decoration = {random steps, amplitude=1pt, segment length=15pt}
        , outer sep = -15pt, inner sep = 0pt, decorate
        , every highlighter, this highlighter ]
        ($(begin highlight)+(0,8pt)$) rectangle ($(end highlight)+(0,-3pt)$) ;
}

\newcommand{\highlight@BeginHighlight}{
  \coordinate (begin highlight) at (0,0) ;
}

\newcommand{\highlight@EndHighlight}{
  \coordinate (end highlight) at (0,0) ;
}

\newdimen\highlight@previous
\newdimen\highlight@current

\DeclareRobustCommand*\highlight[1][]{%
  \tikzset{this highlighter/.style={#1}}%
  \SOUL@setup
  %
  \def\SOUL@preamble{%
    \begin{tikzpicture}[overlay, remember picture]
      \highlight@BeginHighlight
      \highlight@EndHighlight
    \end{tikzpicture}%
  }%
  %
  \def\SOUL@postamble{%
    \begin{tikzpicture}[overlay, remember picture]
      \highlight@EndHighlight
      \highlight@DoHighlight
    \end{tikzpicture}%
  }%
  %
  \def\SOUL@everyhyphen{%
    \discretionary{%
      \SOUL@setkern\SOUL@hyphkern
      \SOUL@sethyphenchar
      \tikz[overlay, remember picture] \highlight@EndHighlight ;%
    }{%
    }{%
      \SOUL@setkern\SOUL@charkern
    }%
  }%
  %
  \def\SOUL@everyexhyphen##1{%
    \SOUL@setkern\SOUL@hyphkern
    \hbox{##1}%
    \discretionary{%
      \tikz[overlay, remember picture] \highlight@EndHighlight ;%
    }{%
    }{%
      \SOUL@setkern\SOUL@charkern
    }%
  }%
  %
  \def\SOUL@everysyllable{%
    \begin{tikzpicture}[overlay, remember picture]
      \path let \p0 = (begin highlight), \p1 = (0,0) in \pgfextra
        \global\highlight@previous=\y0
        \global\highlight@current =\y1
      \endpgfextra (0,0) ;
      \ifdim\highlight@current < \highlight@previous
        \highlight@DoHighlight
        \highlight@BeginHighlight
      \fi
    \end{tikzpicture}%
    \the\SOUL@syllable
    \tikz[overlay, remember picture] \highlight@EndHighlight ;%
  }%
  \SOUL@
}

\makeatother

% Common abbrev. are set as commands to ensure proper spacing after the dot
\newcommand{\ie}{i.e.\@\xspace}
\newcommand{\aka}{a.k.a.\@\xspace}
\newcommand{\Aka}{A.k.a.\@\xspace}
\newcommand{\Ie}{I.e.\@\xspace}
\newcommand{\cf}{cf.\@\xspace}
\newcommand{\Cf}{Cf.\@\xspace}
\newcommand{\eg}{e.g.\@\xspace}
\newcommand{\Eg}{E.g.\@\xspace}
\newcommand{\etal}{et al.\@\xspace}
\newcommand{\etc}{etc.\@\xspace}
\newcommand{\wrt}{w.r.t.\@\xspace}
\newcommand{\Wrt}{W.r.t.\@\xspace}
\newcommand{\mc}{Maven Central\@\xspace}
\newcommand{\latests}{\text{\texttt{LATESTS}\@\xspace}}
\newcommand{\pas}{\text{\texttt{P}\@\xspace}}
\newcommand{\act}{\text{\texttt{A}\@\xspace}}
\newcommand{\latest}{\text{$latest$\@\xspace}}
\newcommand{\notlatests}{\overline{\latests}}%% NOTE, it should be used in Math mode!
\newcommand{\mdg}{MDG\@\xspace}
\newcommand{\mdgl}{$\text{MDG}_L$\@\xspace}
\newcommand{\start}{\texttt{START}\@\xspace}
\newcommand{\snapshot}{\texttt{SNAPSHOT}\@\xspace}
\newcommand{\isPassive}{isPsv}
\newcommand{\orderV}{\displaystyle {<}_{v}}
\newcommand{\orderT}{\displaystyle {<}_{t}}
\newcommand{\lib}{\texttt{LIBS}\@\xspace}
% comment commands for co-authors
\newcommand{\amine}[1]{\mynote{Amine}{#1}}
\newcommand{\cesar}[1]{\mynote{Cesar}{#1}}
\newcommand{\benoit}[1]{\mynote{Benoit}{#1}}
\newcommand{\nicolas}[1]{\mynote{Nicolas}{#1}}
\renewcommand{\todo}[1]{\mynote{TODO}{#1}}


\newcommand{\nbartifacts}{$1,487,956$\@\xspace}
\newcommand{\nblibraries}{$73,653$\@\xspace}

